Subjective Simulation as a Notion of Morphism for Composing Concurrent Resources

Recent approaches to verifying programs in separation logics for concurrency have used state transition systems (STSs) to specify the atomic operations of programs. A key challenge in the setting has been to compose such STSs into larger ones, while enabling programs specified under one STS to be linked to a larger one, without reverification. This paper develops a notion of morphism between two STSs which permits such lifting. The morphisms are a constructive form of simulation between the STSs, and lead to a general and concise proof system. We illustrate the concept and its generality on several disparate examples, including staged construction of a readers/writers lock and its proof, and of proofs about quiescence when concurrent programs are executed without external interference.

==> Makefile <==
all: paper.pdf

paper.pdf: paper.tex abstract.tex intro.tex overview.tex formal.tex rwlock.tex param.tex related.tex conclusions.tex \
           paramdefs.tex model.tex defs.tex references.bib proceedings.bib Makefile \
           acmart.cls 
	echo "\def\draftflag{1}" > flags.tex
	pdflatex paper
	bibtex paper -min-crossrefs=5
	pdflatex paper
	pdflatex paper

# paper.pdf: paper.tex abstract.tex intro.tex overview.tex formal.tex rwlock.tex param.tex related.tex conclusions.tex \
#            paramdefs.tex model.tex defs.tex references.bib proceedings.bib Makefile \
#            acmart.cls 
# 	pdflatex paper
# 	bibtex paper -min-crossrefs=5
# 	pdflatex paper
# 	pdflatex paper


quick:
	pdflatex paper

clean:
	rm -f *~ *.aux *.log *.blg *.dvi *.bm *.vrb *.toc *.nav *.out *.snm *.lof *.lot *.rel *.ps *.bbl paper.pdf flags.tex

zip:    zip paper.zip \
        paper.tex abstract.tex intro.tex overview.tex formal.tex rwlock.tex param.tex related.tex conclusions.tex \
        paramdefs.tex model.tex defs.tex references.bib proceedings.bib Makefile \
        acmart.cls 


